SYGMA: Stellar Yields for Galactic Modeling Applications

The stellar yields for galactic modeling applications (SYGMA) code is an open-source module that models the chemical ejecta and feedback of simple stellar populations (SSPs). It is intended for use in hydrodynamical simulations and semi-analytic models of galactic chemical evolution. The module includes the enrichment from asymptotic giant branch (AGB) stars, massive stars, SNIa and neutron-star mergers. An extensive and extendable stellar yields library includes the NuGrid yields with all elements and many isotopes up to Bi. Stellar feedback from mechanic and frequency-dependent radiative luminosities are computed based on NuGrid stellar models and their synthetic spectra. The module further allows for customizable initial-mass functions and supernova Ia (SNIa) delay-time distributions to calculate time-dependent ejecta based on stellar yield input. A variety of r-process sites can be included. A comparison of SSP ejecta based on NuGrid yields with those from Portinari et al. (1998) and Marigo (2001) reveals up to a factor of 3.5 and 4.8 less C and N enrichment from AGB stars at low metallicity, a result we attribute to NuGrid's modeling of hot-bottom burning. Different core-collapse supernova explosion and fallback prescriptions may lead to substantial variations for the accumulated ejecta of C, O and Si in the first $10^7\, \mathrm{yr}$ at $Z=0.001$. An online interface of the open-source SYGMA module enables interactive simulations, analysis and data extraction of the evolution of all species formed by the evolution of simple stellar populations.

==> abstract.tex <==
\begin{abstract}

%\noindent 	
%250 words mnras,apjs

  The stellar yields for galactic modeling applications (\code{SYGMA})
  code is an open-source module that models the chemical ejecta and
  feedback of simple stellar populations (SSPs). It is intended for
  use in hydrodynamical simulations and semi-analytic models of
  galactic chemical evolution. The module includes the enrichment from
  asymptotic giant branch (AGB) stars, massive stars, SNIa and
  neutron-star mergers. An extensive and extendable stellar yields
  library includes the NuGrid yields with all elements and many
  isotopes up to Bi.  Stellar feedback from mechanic and
  frequency-dependent radiative luminosities are computed based on
  NuGrid stellar models and their synthetic spectra. The module
  further allows for customizable initial-mass functions and supernova
  Ia (SNIa) delay-time distributions to calculate time-dependent
  ejecta based on stellar yield input. A variety of r-process sites can be included. 
A comparison of SSP ejecta based on NuGrid yields with those from \cite{portinari:98} and \cite{marigo:01} reveals up to a factor of 3.5 and 4.8 less C and N enrichment from AGB stars at low metallicity, a result we attribute to NuGrid's modeling of hot-bottom burning. Different core-collapse supernova explosion and fallback prescriptions
may lead to substantial variations for the accumulated ejecta of C, O
and Si in the first $10^7\, \mathrm{yr}$ at $Z=0.001$.  An online
interface of the open-source \code{SYGMA} module enables interactive
simulations, analysis and data extraction of the evolution of all
species formed by the evolution of simple stellar populations.

%leads to higher N abundances in the ejecta 
	
\end{abstract}


==> discussion.tex <==
\section{Discussion} \label{s.science3}


\subsection{Comparison with Wiersma et al.}

In order to verify the \code{SYGMA} code we compare the SSP ejecta calculated with \code{SYGMA} with the results presented in W09, 
using the same set of stellar yields as in W09. 
We apply the net yields of AGB star models by M01 and net yields of massive star models
by P98. We modify C, Mg and Fe yields of massive star models by a factor
of 0.5, 2 and 0.5 as in W09. The initial abundance of elements is taken from Table 1 of W09.
We aim to adopt the same chemical evolution parameter as in that work (\tab{tab:ce_parameter}).

\begin{figure*}[!htbp]
\centering
\includegraphics[width=1.\textwidth]{figs/wiersma_fig2.png}
\caption{Fraction of total mass ejected from AGB, massive star and SNe Ia for a SSP at solar metallicity
with yield input from M01P98 (blue, crosses) compared to results extracted from Fig.\ 2 in W09 (red). 
Results are based on the same yield input but different SSP codes.
}
\label{fig:wiersma_fig2}
\end{figure*}

The initial mass range for which yields were ejected is not given W09 and we choose the range from
$\mzams=0.8\msun$ to $\mzams=100\msun$ to match best Fig.\ 2 in W09.
The lower limit is the lowest initial mass of stellar models
to ignite central He and to enter the AGB stage \citep{karakas:11}. 
Stars of lower initial mass are not of relevance due to their long lifetime beyond the Hubble time.

The choice of $M_{\rm mass}$ is not given in W09.  It might be in the transition range from the largest intermediate-mass model of $\mzams=7\msun$ to the smallest massive star model  of $\mzams=9\msun$ of the M01P98 set.
$M_{\rm mass}$  depends on the upper limit of super-AGB stars and their electron-capture SN channel. 
\cite{poelarends:08} estimated $M_{\rm mass}=9.25\msun$ based on their models
of solar metallicity but the threshold might vary with metallicity \citep{doherty:15,doherty:17}.
$M_{\rm mass}$ depends sensitively on the core growth which in turn
depends on the choice of mass loss and efficiency of TDUP in the AGB stage.
\cite{jones:16} found that an increasing convective boundary mixing efficiency 
increases the TDUP efficiency in super-AGB stars and impedes core growth which would increase $M_{\rm mass}$.
Our choice of $M_{\rm mass}$ (\tab{tab:ce_parameter}) agrees best with the accumulated fraction of ejecta of AGB stars, massive stars
and SNe Ia of Fig.\ 2 in W09.

We compare the accumulated fraction of total ejecta of AGB stars, massive stars
and SNe Ia of our SSP model with W09 at solar metallicity (Figure~\ref{fig:wiersma_fig2}).
The uncertainty related to the value of the transition mass $M_{\rm mass}$
translates into a uncertainty of the appearance of the AGB star ejecta and the drop in total massive star ejecta as shown
for  $M_{\rm mass}=7.5\msun$, $8\msun$ and $8.5\msun$ in Figure~\ref{fig:ce_comparisons}.

\begin{figure}[!htbp]
\includegraphics[width=0.47\textwidth]{figs/transition_mass_comparison.png}
\caption{Evolution of fraction of total ejecta for transition masses of $\mzams=7.5\msun$, $\mzams=8\msun$ and $\mzams=8.5\msun$. 
}
\label{fig:ce_comparisons}
\end{figure}

Our prediction of the evolution of C shows up to 10\% less ejecta from intermediate-mass stars compared to W09.
There is a better agreement above $10^{9}\, \mathrm{yr}$ when stars below $\mzams=2\msun$ start ejecting their material.
The N yields increase smoothly with initial mass which leads to a smooth increase of the SSP ejecta similar to W09.
The differences in the C and N evolution could be due to different yield interpolation methods used in the initial mass transition region from AGB to massive stars.
The variations of C and N yields of massive AGB models combined with
different model assumptions might explain the deviation between our results and W09.

\begin{figure*}[!htbp]
\centering
\includegraphics[width=1.\textwidth]{figs/wiersma_fig3.png}
\caption{Elemental ratios of the total ejecta of a SSP at solar metallicity simulated with \code{SYGMA} compared 
to results by W09. All calculations are with yields from M01P98. 
}
\label{fig:wiersma_fig3}
\end{figure*}

The elements O and Si agree very well with W09 (Figure~\ref{fig:wiersma_fig2}).
They are dominantly produced in massive stars within the first $3\times10^7\, \mathrm{yr}$ and 
the dependence of the massive star ejecta on initial mass cannot be analyzed through Figure~\ref{fig:wiersma_fig2} due to its axis limits.
The evolution of Fe ejecta of massive stars and SNe Ia are qualitative similar while the differences are of similar magnitude as for C.
The contribution from AGB stars stems from the initial, unprocessed material and there is good agreement between our result and W09.

We compare the evolution of [C/Fe], [N/Fe], [O/Fe] and [Si/Fe] with W09 (Figure~\ref{fig:wiersma_fig3}). 
The overall largest differences are found within
the first $\approx2\times10^7\, \mathrm{yr}$ where [C/Fe] from our SSP model is over $0.4\, \mathrm{dex}$ larger than W09.
During this time the enrichment originates only from massive stars. The stellar yields
of the massive star models span $1.7\, \mathrm{dex}$ in [C/Fe] over the initial mass range. 

[C/Fe] in the SSP ejecta is very sensitive to the upper limit of the IMF yield range.
A decrease of the upper IMF yield limit from our best value matching W09 of $\mzams=100\msun$ down to $\mzams=30\msun$ 
results in a better agreement with the first value of [C/Fe] = 0.7 of W09 (Figure~\ref{fig:ce_comparisons2}).
But later in the evolution [C/Fe] drops by about $0.5\, \mathrm{dex}$ below the results of W09. The choice of the upper limit
of the IMF as W09 together with the same interpolation of C and Fe with initial mass as W09 could result in a better
agreement.
[N/Fe], [O/Fe] and in particular [Si/Fe] of the yields vary less strongly with initial mass which might explain the better agreement with W09 (Figure~\ref{fig:wiersma_fig3}).

\begin{figure}[!htbp]
\centering
\includegraphics[width=0.47\textwidth]{figs/upper_imf_comparison.png}
\caption{Evolution of [C/Fe] for upper boundaries of $\mzams=30\msun$, $\mzams=65\msun$ and $\mzams=100\msun$ up to which yields are applied.
}
\label{fig:ce_comparisons2}
\end{figure}

\begin{figure*}[!htbp]
\centering
\includegraphics[width=1.\textwidth]{figs/wiersma_fig2_style_yield_comparison.png}
\caption{Fraction of total mass ejected from AGB, massive star and SNe Ia for a \code{SYGMA} SSP at solar metallicity
with NuGrid yield (blue, crosses) and yields from M01P98 (red).
}
\label{fig:wiersma_fig2_yield_comparison}
\end{figure*}

To compare the effect of SSP assumptions and yield input we distinguish between the same SSP assumptions but different yields input (NuGrid vs M01P98, Figure~\ref{fig:wiersma_fig2_yield_comparison})
and different SSP assumptions with same yield input (Figure~\ref{fig:wiersma_fig2}). %case A
Early on when AGB stars eject matter there is a larger disagreement in the evolution of C due to different chemical evolution assumptions 
while at later times is is due to different yield input. 
The evolution of N, O and Si differ the most for different yield input which is likely due to the treatment of fallback in the stellar models. 
Fe differs stronger with the change in chemical evolution assumptions than with change in yield input.
The same SNIa yields are applied in both sets which results in a good agreement when the same chemical evolution assumptions are applied.
Overall we find that differences in yield input is more relevant than the differences in the SSP implementation

\subsection{Impact of Mass-cut Prescriptions} \label{s.science5}

The composition of SSP ejecta depends on the choice of the CCSN prescription and
fallback of the massive star models. NuGrid provides stellar yields with two different explosion prescriptions 
(yield set NuGrid$_{\rm d}$, yield set NuGrid$_{\rm r}$, \tab{tab:yieldcompilations})  based
on the convective-enhanced neutrino-driven engine and we discuss the impact of these prescriptions for SSPs at $Z=0.02$ and $Z=0.001$ \citep[e.g.][F12]{fryer:07,fryer:12}.
On a short timescale the rapid-convection engine 
provides enough energy for a successful explosion. 
The delayed-convection explosion requires longer times to deposit enough energy to explode which results in more fallback
and larger remnants for stellar models of $Z=0.02$ and $Z=0.001$ (Figure~\ref{fig:masscuts}). The $25\msun$, $Z=0.02$ model is an exception  to this statement.
The remnant mass in the delayed explosion increases with initial mass while the remnant mass for the rapid
explosion peaks strongly around $\mzams=24\msun$. The latter results in the large remnant mass of $15.5\msun$ for
our stellar model with $\mzams=25\msun$.
According to F12 this stellar model collapses directly into a BH which results the total mass at collapse as the remnant mass (Figure~\ref{fig:masscuts}).
 %In stellar models and both explosion prescriptions fallback increases with initial mass.
\begin{figure}[!htbp]
\centering
\includegraphics[width=0.47\textwidth]{figs/mass_cuts_all.png}
\caption{Remnant masses based on stellar models of $Z=0.02$
and $Z=0.001$ from NuGrid and calculated the delayed and rapid explosion prescriptions.
%\href{https://github.com/NuGrid/NuPyCEE/blob/master/DOC/Papers/SYGMA_paper/Section4.2.ipynb}{Online Access}.
}
\label{fig:masscuts}
\end{figure}

We compare the impact of the two fallback prescriptions on the massive star ejecta of
SSPs of $1\msun$ for $Z=0.02$ and $Z=0.001$ (Figure~\ref{fig:ssp_fallback}).
\begin{figure*}[!htbp]
\centering
\includegraphics[width=1.\textwidth]{figs/ssp_delay_rapid_yields.png}
\caption{Accumulated ejecta of massive stars of NuGrid yields at $Z=0.02$ and $Z=0.001$ computed with
the delayed and rapid CCSN fallback prescription, for an SSP of $1\msun$.
}
\label{fig:ssp_fallback}
\end{figure*}
The SSP ejecta of C, O and Si differ more between the fallback prescriptions at $Z=0.02$ than at $Z=0.001$ due 
to the BH formation after the rapid explosion of the stellar model with $\mzams=25\msun$ at $Z=0.001$. 
This prevents the ejection of the Si, O and C shell.
Similar amounts of Fe fall back onto the remnant with both explosion prescriptions due to the deep location of the Fe core.
The SSP ejecta of Fe show only smaller differences.
The ejection of elements of the SSP at $Z=0.001$ agree well except for Fe.
Small amounts of fallback in the rapid explosion of the stellar model with $\mzams=20\msun$ and a sufficient large Fe core
result in the ejection of a thin layer of the Fe core which boosts the amount of Fe SSP ejecta. Within the first $1.3\times10^7\, \mathrm{yr}$
ten times more Fe is ejected with the rapid explosion compared to the delayed explosion. The expected 
range of explosion delay times (F12) could lead to large variations in Fe enrichment in the early universe.

The rapid explosion models match better the observed gap between NS and BH remnants than the
delayed models even though the gap might be sparsely populated (references in F12). 
Delayed explosions produce more fallback BHs, in particular at low mass and
yield a larger fraction of low-mass BHs formed with a SN explosion.
The latter can explain the observed BH systems which indicate a natal kick (F12).
Fallback is also relevant to produce the weak supernova \citep{valenti:09} which are believed to be observed (F12). 
While the yield sets with the delayed and rapid CCSN explosion prescription are 
valid to use we recommend yields with the delayed explosion prescription in chemical evolution models.
F12 argues that both extremes might be necessary to explain all SN observations. 
We combine yields of the delayed and rapid explosions to take
into account explosions on short and long timescale and provide a yield table which contains as a mixture half of the yields of each prescription (yield set NuGrid$_{\rm d/r/m}$, \tab{tab:yieldcompilations}).


